Mid-Infrared Evidence for Accelerated Evolution in Compact Group Galaxies

Compact galaxy groups are at the extremes of the group environment, with high number densities and low velocity dispersions that likely affect member galaxy evolution. To explore the impact of this environment in detail, we examine the distribution in the mid-infrared (MIR) 3.6-8.0 micron colorspace of 42 galaxies from 12 Hickson compact groups in comparison with several control samples, including the LVL+SINGS galaxies, interacting galaxies, and galaxies from the Coma Cluster. We find that the HCG galaxies are strongly bimodal, with statistically significant evidence for a gap in their distribution. In contrast, none of the other samples show such a marked gap, and only galaxies in the Coma infall region have a distribution that is statistically consistent with the HCGs in this parameter space. To further investigate the cause of the HCG gap, we compare the galaxy morphologies of the HCG and LVL+SINGS galaxies, and also probe the specific star formation rate (SSFR) of the HCG galaxies. While galaxy morphology in HCG galaxies is strongly linked to position with MIR colorspace, the more fundamental property appears to be the SSFR, or star formation rate normalized by stellar mass. We conclude that the unusual MIR color distribution of HCG galaxies is a direct product of their environment, which is most similar to that of the Coma infall region. In both cases, galaxy densities are high, but gas has not been fully processed or stripped. We speculate that the compact group environment fosters accelerated evolution of galaxies from star-forming and neutral gas-rich to quiescent and neutral gas-poor, leaving few members in the MIR gap at any time.

==> gapslope.tex <==
\ProvidesFile{gapslope.tex}%
 [2003/12/12 5.2/AAS markup document class]%

\begin{deluxetable}{ccc}
\tablewidth{0pt}
\tablecaption{CDF Slopes in Gap Region\label{gapslope}}
\tablehead{
\colhead{} &	\multicolumn{2}{c}{Slope} \\
\colhead{Sample} &	\colhead{Cropped} &	\colhead{Uncropped}}
\startdata
HCG		&	0.104	&	\nodata \\
LVL+SINGS	&	0.732	&	0.743 \\
LVL+SINGS (culled)	&	0.896	&	0.883 \\
Interacting	&	\nodata	&	\nodata \\
Coma (center)	&	0.600	&	0.518 \\
Coma (infall)	&	0.261	&	0.246 \\
%Interacting	&	0.225	&	sample begins mid-gap \\
%Starburst	&	0.175	&	sample begins mid-gap \\
\enddata
\tablecomments{Slopes of the CDFs of all the samples over the region of the gap in the HCG sample.}
\end{deluxetable}

\endinput
%%
%% End of file `ksone.tex'.


==> hcgsample.tex <==
\ProvidesFile{hcgsample.tex}%
 [2003/12/12 5.2/AAS markup document class]%

%$\log{M_{\ion{H}{1}}}$
\begin{deluxetable}{cccccc}
\tablewidth{0pt}
\tablecaption{HCG Sample\label{hcgsample}}
\tablehead{
\colhead{HCG} &	\colhead{R.A.} &	\colhead{Dec} &	\colhead{D\tablenotemark{a}} &	\colhead{$\log{M_{\mathrm{H \; I}}}$\tablenotemark{b}} &	\colhead{Group Type\tablenotemark{c}} \\
\colhead{} &	\colhead{(J2000)} &	\colhead{(J2000)} &	\colhead{(Mpc)} &	\colhead{($M_\sun$)} &	\colhead{}}
\startdata
02 & 0$^\mathrm{h}$31$^\mathrm{m}$30\fs0 & +8\degr25\arcmin52\arcsec & 136.6 & 10.33 & I \\
%\begin{comment}
07 & 0$^\mathrm{h}$39$^\mathrm{m}$23\fs9 & +0\degr52\arcmin41\arcsec & 56.4 & 9.68 & II \\
16 & 02$^\mathrm{h}$09$^\mathrm{m}$31\fs3 & -10\degr09\arcmin31\arcsec & 52.9 & $>$10.42 & I \\
19 & 02$^\mathrm{h}$42$^\mathrm{m}$45\fs1 & -12\degr24\arcmin43\arcsec & 57.3 & 9.31 & II \\
22 & 03$^\mathrm{h}$03$^\mathrm{m}$31\fs3 & -15\degr40\arcmin32\arcsec & 36.1 & 9.13 & II \\
31 & 05$^\mathrm{h}$01$^\mathrm{m}$38\fs3 & -04\degr15\arcmin25\arcsec & 54.5 & 10.35 & I \\
42 & 10$^\mathrm{h}$00$^\mathrm{m}$21\fs8 & -19\degr38\arcmin57\arcsec & 53.3 & 9.40 & III \\
48 & 10$^\mathrm{h}$37$^\mathrm{m}$45\fs6 & -27\degr04\arcmin50\arcsec & 37.7 & 8.52 & III \\
59 & 11$^\mathrm{h}$48$^\mathrm{m}$26\fs6 & +12\degr42\arcmin40\arcsec & 54.1 & 9.49 & II \\
61 & 12$^\mathrm{h}$12$^\mathrm{m}$24\fs9 & +29\degr11\arcmin21\arcsec & 52.1 & 9.96 & I \\
62 & 12$^\mathrm{h}$53$^\mathrm{m}$08\fs1 & -09\degr13\arcmin27\arcsec & 54.9 & $<$9.06 & III \\
90 & 22$^\mathrm{h}$02$^\mathrm{m}$06\fs0 & -31\degr55\arcmin48\arcsec & 32.3 & 8.66 & III \\
%\end{comment}
\enddata
\tablenotetext{a}{Group distance taken from NED. The cosmology used was $H_0=73\;{\rm km\,s^{-1}\,Mpc^{-1}}$, $\Omega_{matter}=0.27$, and $\Omega_{vacuum}=0.73$.}
\tablenotetext{b}{\ion{H}{1} masses from \citet{verdes01}, with the exception of HCG 90, provided by J. Hibbard 2006, private communication.}
\tablenotetext{c}{Group type discussed in \S\ref{hcgobs}. Type I = \ion{H}{1}-rich, Type III = \ion{H}{1}-poor.}
%% You can append references to a table using the \tablerefs command.
%\tablerefs{(1) Barbuy, Spite, \& Spite 1985; (2) Bond 1980; (3) Carbon et al. 1987; (4) Hobbs \& Duncan 1987; (5) Gilroy et al. 1988: (6) Gratton \& Ortolani 1986; (7) Gratton \& Sneden 1987; (8) Gratton \& Sneden (1988); (9) Gratton \& Sneden 1991; (10) Kraft et al. 1982; (11) LCL, or Laird, 1990; (12) Leep \& Wallerstein 1981; (13) Luck \& Bond 1981; (14) Luck \& Bond 1985; (15) Magain 1987; (16) Magain 1989; (17) Peterson 1981; (18) Peterson, Kurucz, \& Carney 1990; (19) RMB; (20) Schuster \& Nissen 1988; (21) Schuster \& Nissen 1989b; (22) Spite et al. 1984; (23) Spite \& Spite 1986; (24) Hobbs \& Thorburn 1991; (25) Hobbs et al. 1991; (26) Olsen 1983.}
%\tablecomments{RA, Dec, Type, and Group Type from \citet{hcgs}. D and \ion{H}{1} Mass from Amanda's spreadsheet, unless noted. Then from \citep{leon98}.}
\end{deluxetable}

\endinput
%%
%% End of file `hcgtable.tex'.


==> ksone.tex <==
\ProvidesFile{ksone.tex}%
 [2003/12/12 5.2/AAS markup document class]%

\begin{deluxetable}{cccccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{Single-Distribution KS Test\label{ksone}}
\tablehead{
\colhead{} &	\multicolumn{3}{c}{Cropped} &	\multicolumn{3}{c}{Uncropped} &	\colhead{} \\
\cline{2-7}  \\
\colhead{Sample} &	\colhead{N} &	 \colhead{D} &	\colhead{$\alpha$} &	\colhead{N} &	 \colhead{D} &	\colhead{$\alpha$} &	\colhead{Consistent w/Uniform}}
\startdata
HCG	 &	\nodata	& \nodata	& \nodata & 41 & 0.333 & $3.27\times10^{-4}$ & reject \\
LVL+SINGS &	88	& 0.199	& $3.00\times10^{-3}$ & 90 & 0.179 & $9.35\times10^{-3}$ & do not reject \\
LVL+SINGS (culled) &	67	& 0.236	& $1.72\times10^{-3}$ & 68 & 0.238 & $1.37\times10^{-3}$ & do not reject \\
Interacting &	57	& 0.376	& $3.12\times10^{-7}$ & 58 & 0.375 & $2.79\times10^{-7}$ & reject \\
Coma (center) &	128	& 0.622 & $1.60\times10^{-43}$ & 155 & 0.378 & $1.96\times10^{-19}$ & reject \\
Coma (infall) &	48	& 0.482	& $5.60\times10^{-10}$ & 51 & 0.479 & $1.91\times10^{-10}$ & reject \\
\enddata
\tablecomments{The model uniform distribution covers only the range where galaxies are located, and is different for each sample.}
\end{deluxetable}

\endinput
%%
%% End of file `ksone.tex'.


==> kstwo.tex <==
\ProvidesFile{kstwo.tex}%
 [2003/12/12 5.2/AAS markup document class]%

\begin{deluxetable}{ccccccccc}
\tabletypesize{\scriptsize}
%\rotate
\tablewidth{0pt}
\tablecaption{Two-Distribution KS Test\label{kstwo}}
\tablehead{
\colhead{} &	\multicolumn{3}{c}{Cropped} &	\multicolumn{3}{c}{Uncropped} &	\colhead{} &	\colhead{} \\
\cline{2-7}  \\
\colhead{Sample} &	\colhead{$\mathrm{N_{HCGs}}$} &	 \colhead{D} &	\colhead{$\alpha$} &	 \colhead{$\mathrm{N_{HCGs}}$} &	 \colhead{D} &	\colhead{$\alpha$} &	\colhead{Consistent w/HCGs} &	\colhead{Reason}}
\startdata
LVL+SINGS		& 38 & 0.406 & $4.24\times10^{-4}$ & 41 & 0.399 & $3.42\times10^{-4}$ & likely reject & a,b\\
LVL+SINGS (culled)		& 36 & 0.413 & $8.74\times10^{-4}$ & 41 & 0.429 & $2.11\times10^{-4}$ & likely reject & a,b\\
Interacting	& 21 & 0.459 & $3.52\times10^{-3}$ & 41 & 0.574 & $3.11\times10^{-7}$ & reject & b,c\\
Coma (center)	& 40 & 0.414 & $7.87\times10^{-5}$ & 41 & 0.441 & $9.01\times10^{-6}$ & reject & a,c\\
Coma (infall)	& 38 & 0.292 & 0.059 & 41 & 0.292 & 0.047 & do not reject & c
\enddata
\tablecomments{Cropped covers only the region of colorspace that galaxies from both samples occupy. Uncropped covers the entire region of colorspace that galaxies from either sample occupy. Qualitative reasons for inconsistency: (a) no gap; (b) fundamentally different; (c) covers different range in colorspace, if uncropped.}
\end{deluxetable}

\endinput
%%
%% End of file `kstwo.tex'.

